Nested Learning For Multi-Granular Tasks

Standard deep neural networks (DNNs) are commonly trained in an end-to-end fashion for specific tasks such as object recognition, face identification, or character recognition, among many examples. This specificity often leads to overconfident models that generalize poorly to samples that are not from the original training distribution. Moreover, such standard DNNs do not allow to leverage information from heterogeneously annotated training data, where for example, labels may be provided with different levels of granularity. Furthermore, DNNs do not produce results with simultaneous different levels of confidence for different levels of detail, they are most commonly an all or nothing approach. To address these challenges, we introduce the concept of nested learning: how to obtain a hierarchical representation of the input such that a coarse label can be extracted first, and sequentially refine this representation, if the sample permits, to obtain successively refined predictions, all of them with the corresponding confidence. We explicitly enforce this behavior by creating a sequence of nested information bottlenecks. Looking at the problem of nested learning from an information theory perspective, we design a network topology with two important properties. First, a sequence of low dimensional (nested) feature embeddings are enforced. Then we show how the explicit combination of nested outputs can improve both the robustness and the accuracy of finer predictions. Experimental results on Cifar-10, Cifar-100, MNIST, Fashion-MNIST, Dbpedia, and Plantvillage demonstrate that nested learning outperforms the same network trained in the standard end-to-end fashion.

==> supplementaryMaterial.tex <==

% ====================================================== %
\appendix
\counterwithin{table}{section}
\counterwithin{figure}{section}
\section{Additional examples}\label{app:sec:more_examples}
\counterwithin{table}{section}
\counterwithin{figure}{section}
% ====================================================== %
\begin{figure}[htp]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/examples.png}
    \caption{These results complement Figure~\ref{fig:example1}. The output of a standard (end-to-end) DNN and our proposed nested learning version are compared. 
    %
    On the left, we show clean images from the test set of CIFAR-10 dataset, on the right, the same examples but blured. Next to each image our prediction (for the fine, middle, and coarse level) and the prediction of a standard (end-to-end) DNN are displayed. 
    %
    Both DNNs share the same architecture and their performance is compared on Table~\ref{tab:cifar10_202020vs20} (rows  ``end-to-end, $|\mathcal{D}_3|=\frac{3N}{2}$'' and ``nested, $|\mathcal{D}_{1,2,3}|=N$''). 
    %
    As shown in Table~\ref{tab:cifar10_202020vs20}, while the performance of both networks is similar on clean data (i.e., data that match the train distribution), learning nested representations significantly boost models robustness and mitigates overconfident predictions.}
    \label{app:fig:more_examples_usVSstandard}
\end{figure}

\section{Combination methods}\label{app:sec:combination}
\counterwithin{table}{section}
\counterwithin{figure}{section}
% ====================================================== %
Combining multiple classifiers is a standard approach in machine learning. 
%
However, most approaches combine similar outputs and are not designed for the specific problem of nested learning. 
% 
We compared standard combination methods and the proposed calibration-based combination strategy.
% ---

Combination methods can be classified into two categories. 
%
First those that combine classifiers predicted label, in this case, classifier outputs are considered as one-hot encoding vectors. 
% 
For example, the \emph{Majority Vote (MA)} which consists in aggregating the decision of multiple classifiers and selecting the candidate that receives more votes.
%
The second category, combine classifiers continuous score outputs (rather than discrete labels).
%
As we show in the following, the second class of methods are more suitable for the combination of nested outputs. 
% ---

%For example, suppose that given an input sample $x$, the classifier outputs an estimations of the probability associated to each coarse, middle, and fine label: $P_{\hat{Y}_1}$, $P_{\hat{Y}_2}$, and $P_{\hat{Y}_3}$.
For example, given an input sample, a calibrated classifier provides an approximation of the probability associated to each coarse, middle, and fine labels.
%
In order to apply standard combination methods, we must map the coarse and intermediate predictions into a fine prediction and vice-versa. 
%
To this end, we assume coarse predictions have no information about the finer levels, and therefore, the probability of a coarse node is equally distributed across the fine nodes associated to it. 
% ---

Once probabilities associated to coarse levels are propagated to the fine levels and vice-versa, we can combine them using the \emph{mean} or the \emph{product} rule as described in \cite{kuncheva_2004}. 
%
Table~\ref{app:tab:combinationsMNIST101010} shows the result of combining nested outputs with standard combination methods and our strategy described in Section~\ref{subsec:CombinationOfOutputs}. 
\begin{table}[htp]
    \scriptsize
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|}
        \hline
        Distortion & Without comb.&  Ours & Coarse \& Fine& Mean &  Product & MV \\
        \hline
        Original     & \textbf{98.8} & 98.6 & 98.7 & 98.7 & 98.7 & 98.5 \\
        Distortion 2 & 80.8 & \textbf{82.8} & 82.1 & 82.2 & 82.4 & 80.1 \\
        Distortion 4 & 45.8 & \textbf{50.6} & 49.6 & 48.6 & 49.6 & 47.5  \\
      \hline
\end{tabular}
    \caption{\footnotesize Comparison of the fine accuracy for different combination techniques. The model is trained on MNIST dataset with $|\mathcal{D}_1|=|\mathcal{D}_2|=|\mathcal{D}_3|= 6000$ }
    \label{app:tab:combinationsMNIST101010}
\end{table}

% ====================================================== %
\section{Implementation Details}\label{app:sec:implem_details}
\counterwithin{table}{section}
\counterwithin{figure}{section}
% ====================================================== %
%
\subsection{Architecture}
\textbf{MNIST, Fashion-MNIST, CIFAR 10, Plantvillage.}
%
The architecture of our model is presented in Figure~\ref{app:fig:mnist_architecture}.
%
We used the same architecture for MNIST and Fashion-MNIST as the images have the same size and number of channels. 
%
For CIFAR10 and the Plantvillage data, the architecture of our model is very similar but with an increased depth of the convolutional filters.
%
We report the number of parameters for each model in Table~\ref{app:tab:params}.
Classifying images from CIFAR10 is indeed a harder problem than classifying images from MNIST or Fashion-MNIST, and therefore, it requires a model with more parameters.
\begin{table}[]
    \centering
    \scriptsize
    \begin{tabular}{|c||c|c|c|c|c|c|}
         \hline
         Dataset & MNIST & F-MNIST & Cifar 10& PlantVillage& DBPEDIA & CIFAR 100 \\
         \hline
         parameters& $5.2 \times10^4$ &$5.2 \times 10^4$&$ 6.3 \times 10^5$ &$2.4 \times 10^5$ & $4.2 \times 10^5 $ & $1.5 \times 10^6$\\
         \hline
    \end{tabular}
    \caption{Number of parameters for each nested model.}
    \label{app:tab:params}
\end{table}
%
The architecture we use is an adaptation of the U-Net \cite{Unet} designed to fit our proposed framework of nested information bottlenecks.  
%
The U-Net is indeed a good starting point, as it meets most of the criteria that we presented in Section \ref{sec:Theory}. 
%
First, it consists of a convolutional network that enforces a bottleneck representation. 
%
Second, it presents skip connections that allow information from the input to flow to deeper components of the network. 

We also added Batch-Normalization (BN) layers after every convolutional filters in order to achieve a faster convergence. BN is very helpful to mitigate the vanishing gradient phenomenon. Also, since it introduces randomness during training, BN acts as a regularization. Classic L1 regularization was shown to be similar to BN in \cite{luo2018towards}, while including BN layers also improves training speed and stability as explained by \cite{santurkar2018does}.   
%
\begin{figure}[t]
    \centering
    \includegraphics[width = 0.6\textwidth]{figures/mnist_architecture.png}
    \caption{\footnotesize Architecture of our CNN for both Fashion-MNIST and MNIST. 
    %
    This model is an adaptation of the U-Net network \cite{Unet} designed to fit our nested learning framework. 
    %
    The blue boxes represent the features extracted by convolutional layers. 
    %
    We perform a global average pooling rather than a flattening to decrease the number of parameters. 
    %
    After the global average pooling, the feature vector is normalized with respect to the L2 norm (instance normalization layer).
    %
    The normalized features are followed by fully connected layers to compute the final output. 
    %
    The model used to test CIFAR10 set is very similar but has convolutional layers with more kernels to handle this (sightly more complex) task.}\label{app:fig:mnist_architecture}
\end{figure}
% --- 

\noindent\textbf{DBPEDIA.} The architecture for the text data is presented in Figure \ref{app:fig:nlp_architecture_framework}. It is made of three important blocks: a preprocessing operation, a convolutional core, and task-specific layers. The preprocessing consists of a classic data cleaning and lemmatization. It is followed by an embedding to a (200,100) matrix using GloVe \cite{pennington2014glove}. Each line of this matrix corresponds to a vector word embedding of size 100. We pad or truncate articles to a fixed length of 200 to ease the implementation. This embedding is passed to a convotutional core, shown in yellow in Figure \ref{app:fig:nlp_architecture_framework}, which is similar to the U-Net, except that it is one dimensional. 
The intermediate features are passed to the task specific layers. Those layers are made of Bi-directional LSTMS and fully connected layers. Bi-directional LSTMs were shown to be particularly efficient for text classification and other Natural Language Processing tasks \cite{huang2015bidirectional}.
\begin{figure}[htp]
    \centering
    \includegraphics[width = 0.9\textwidth]{eccv2020kit/figures/nlp_schema.pdf}
    \caption{Preprocessing and architecture for the DBPEDIA model. The convolutional trunk is very similar to the one of a U-Net \cite{Unet}. It is associated to LSTM layers which are particularly suited for text data. The classification layers are fully connected layers. }
    \label{app:fig:nlp_architecture_framework}
\end{figure}

\noindent\textbf{CIFAR-100.} The architecture for the CIFAR100 dataset is presented in Figure~\ref{app:fig:cifar100_architecture}. This architecture is inspired by both the U-Net \cite{Unet} and the Densenet \cite{huang2017densely}. Dense net takes a step further in using residual connections by creating densely connected blocks. Those blocks are a sequence of convolution+batch normalization+ReLU layers applied to a concatenation of all the previously extracted features.
%
To get a coarse prediction we use the classic form of a densenet with three dense blocks, a global average pooling layer and a fully connected layer with 20 outputs . Then we upsample the features encoded by the last dense block and concatenate them with the features encoded by the previous dense block. These feature maps are then passed through a dense block which leads to a second average pooling layer and a fully connected layer of 100 outputs.
%
In our architecture, each dense block has the same parameters: 12 layers per block with a growth rate (depth) of 12, with bottleneck and compression layers (BC).  
%
\begin{figure}[htp]
    \centering
    \includegraphics[width = 0.6\textwidth]{eccv2020kit/figures/cifar100_architecture.pdf}
    \caption{Architecture of our model for CIFAR-100 dataset.  This architecture is inspired by both the U-Net \cite{Unet} and the Densenet \cite{huang2017densely}.}
    \label{app:fig:cifar100_architecture}
\end{figure}
% ---

\subsection{Training}
%
We train the proposed nested models in an iterative fashion; First, we optimize the weights for the coarse prediction with the samples that are only coarsely annotated (freezing the remaining weights).
%
Then, we optimize the weights up to the intermediate output with the training samples with coarse and intermediate annotations.
%
This process is repeated for each level until we reach the finer level and the entire network is trained. 
%
Each training step is performed using ADAM optimizer with a specific learning rate. For example, for problems with three nested levels we set the learning rate as: $2\times10^{-3}$ for the first step, $1\times10^{-3}$ for the second, and $5\times10^{-4}$ for the final step.
%
We stop the training of each level when stagnation of the validation loss is observed.
% ---

\subsection{Calibration} 
%
The calibration consists of two main steps. First a ``rejection'' class is modeled using an uniform distribution on the latent space. 
%
This models out-of-distribution samples and mitigates overconfident predictions on portions of the feature space where no training data is observed. 
% 
The second step consists of temperature scaling to convert output scores into approximations of class probabilities. 
% ---
\\

\noindent\textbf{The ``rejection'' class.} 
%
For every level of granularity $i$ and for every sample of the training dataset, we store the normalized outputs of the global averaging layer (GAP) in a dataset $D_i$. 
%
The samples have size $s_i$ and are normalized with respect to the L2 norm, therefore, they live in $\mathcal{B}^{s_i}(0,1)$, the unitary sphere in $\mathbb{R}^{s_i}$ centered at zero. 
%
We randomly sample $n_i$ new instances from an uniform distribution in $\mathcal{B}^{s_i}(0,1)$. These samples (associated to a new ``rejection'' class) are aggregated to $D_i$ and the fully connected layers fine tuned.\footnote{To this end, we used ADAM optimizer with a learning rate of $10^{-3}$.} 
%
Naturally, the larger $|D_i|$ and $s_i$, the larger $n_i$ should be.
%
We set $n_i \propto |D_i| \times \mathcal{S}(s_i)$, where $\mathcal{S}(s_i)$ is the area of the hypersphere of unitary radius in the $s_i$-dimensional space.  
%
Figure~\ref{app:fig:calib_toy} illustrates for a one dimensional toy example how the proposed ideas provide an efficient solution to reduce outputs overconfidence on out-of-distribution input samples.
%
\begin{figure}[h]
\centering     %%% not \center
\subfigure[]{\label{fig:a}\includegraphics[width = 0.32\textwidth]{figures/distribution.png}}
\subfigure[]{\label{fig:b}\includegraphics[width = 0.32\textwidth]{figures/overc.png}}
\subfigure[]{\label{fig:c}\includegraphics[width = 0.32\textwidth]{figures/conf.png}}
\caption{\footnotesize One dimensional toy example that illustrates the problem of prediction overconfidence for input samples that are far from the training distribution. 
%
In this example, two classes (``1'' and ``0'') are considered and we assume that the input $x\sim X$ is  one-dimensional. (a) illustrates the empirical distribution of each class (on green $P(X|Y=1)$ and yellow $P(X|Y=0)$).
%
In addition, we illustrate (blue distribution) the uniform distribution from which we sample synthetic training instances associated to the ``rejection'' class. 
%
Figure (b) shows the confidence output associated to the class ``1'' and ``0'' for different values of $x$, for a model trained only on the original data (standard approach). 
%
Figure (c) illustrates the output of the same DNN trained with the samples associated to the classes ``1'' and ``0'' plus the synthetic samples from the ``rejection'' class.}\label{app:fig:calib_toy}
\end{figure}
% ---
\\

\noindent\textbf{Temperature scaling.} 
%
Temperature scaling improves calibration by converting arbitrary score values into an approximation of class probabilities. 
%
As explained in Section \ref{subsec:Scores_calibration}, we  minimize the empirical ECE metric over the validation set, composed of 5000 unseen samples for all the dataset we tested our method on.
%
To find the optimal temperature $T$, we compute the ECE over $50$ values between $1$ and $3$ and select the one for which the ECE is minimized. 
%
If $T=1$ the model is already well calibrated. 
%
On all our experiments, the minimal ECE value was always reached for $T$ values strictly lower than 3. 
% ---
% ====================================================== %
\section{Dataset taxonomies}\label{app:sec:label_grouping}
\counterwithin{table}{section}
\counterwithin{figure}{section}
\noindent{\textbf{Creating an artificial taxonomy for MNIST, Fashion-MNIST, CIFAR-10.}}
% ====================================================== %
%
To group fine labels into a meaningful nested structure, we first train a shallow neural network and classify images into the fine classes. 
%
Then we used the confusion matrix $M$ associated to this auxiliary classifier to establish which classes are closer to each other. 
Note that this is done here for illustrating our proposed nested framework, other datasets already provide a natural taxonomy.
This way the levels of the nested structure can also have semantic meaning. But as demonstrated in the paper, even without explicit prior taxonomy, this type of nested structure improves performance for all levels.
% ---

For MNIST and Fashion-MNIST for example, we wanted to group the labels in $2$ coarse categories which also contained $2$ intermediate categories. 
%
To this end, we find the permutation $\sigma$ applied to both the rows and columns of $M$, such that the non-diagonal $5\times5$ matrices of $M$ had the lowest possible L1-norm. 
%
We iterate this process to find the intermediate categories.
%
It is computationally hard to go through all the permutations, therefore, we follow the ideas proposed in \cite{Behrisch:2016:MRM:3071534.3071595} to perform matrix reordering with a reduced complexity.
% ---

Figure \ref{app:fig:taxonomies} presents the groups of labels we obtained for MNIST, Fashion-MNIST, and CIFAR10. 
%
Our results show natural and intuitive taxonomies, see e.g., how MNIST digits are grouped according to a natural shape-oriented similarity, with 3 and 8 in the same intermediate class for example. A vertical left occlusion will force a standard DNN to pick between the two (or make a mistake outside this group), while obviously the correct answer is ``a 3 or an 8'' since there is no information for the fine class.
% 
\begin{figure}[h]
\centering     %%% not \center
\subfigure[Taxonomy obtained for MNIST]{\includegraphics[width = 0.32\textwidth]{figures/digit_taxonomy.png}}
\subfigure[Taxonomy obtained for Fashion-MNIST]{\includegraphics[width = 0.32\textwidth]{figures/fashion_mnist_taxonomy.png}}
\subfigure[Taxonomy obtained for CIFAR10]{\includegraphics[width = 0.32\textwidth]{figures/cifar10_taxonomy.png}
}
\caption{\footnotesize Nested groups obtained by minimizing the non-diagonal components on the confusion matrix of an auxiliary simple classifier.}\label{app:fig:taxonomies}
\end{figure}

\noindent{\textbf{Taxonomies for CIFAR-100, DBPEDIA, and Plantvillage.}} 
%
Those datasets are already annotated following a nested taxonomy. CIFAR 100 is a dataset of small natural images of different objects. The labels are organized in 20 coarse classes (e.g., flower), each of them corresponding to 5 fine classes (e.g., orchids, poppies, roses, sunflowers, and tulips).
%
DBPEDIA is a large dataset of articles of wikipedia organized in a three level nested taxonomy. There are 9 coarse classes, 70 middle classes, 219 fine classes. For instance, an article of the Mugdock Castle near Glasgow, is labeled with the triplet (Place, Building, Castle).
%
Finally, Plantvillage dataset contains images of healthy and sick leaves from different species. The labels are not multi-granular. However the labels can be split in a natural nested taxonomy. In our framework, the coarse label corresponds to the species of the leaf ; the intermediate label corresponds to the binary label: healthy or sick . Finally, the fine labels corresponds to what sickness the plant has. Here are some examples of possible labels : (Apple, Apple healthy, Apple healthy), (Tomato, Tomato sick, Tomato Bacterial Spot), etc. By redefining the annotations in that fashion, we have 14 coarse classes, 23 middle classes, and 38 fine classes.
% ---------------------------

\newpage
\section{Additional experiments}\label{app:sec:additional_experiments}
\counterwithin{table}{section}
\counterwithin{figure}{section}
% ====================================================== %
\subsection{Additional results for Fashion MNIST and MNIST}
\begin{table}[ht]
\begin{center}
\hspace{-5mm}
    \scriptsize
    \begin{tabular}{|c|c|c|c|c|c|c|}
    \hline
        ind & method & Original & Distortion 1 &  Distortion 2 &  Distortion 3 &  Distortion 4 \\
          \hline
          \hline
        \multicolumn{7}{|c|}{F-MNIST}\\
          \hline
        J& Coarse (end-to-end), $|\mathcal{D}_3| = \frac{3N}{2}$ & 98.9 / 99.3 & 90.7 / 96.4 &          87.5 / 95.9 &          85.1 / 95.5&          84.0 / 94.7 \\
         K & Coarse (end-to-end), $|\mathcal{D}_3| = N$ &          99.0 / 99.3 &94.5 / 96.9 &          90.1 / 96.1 &          87.3 / 94.9 &      \textbf{85.9} / 94.5 \\
          L  & Coarse (nested), $|\mathcal{D}_{1,2,3}| = N$ & \textbf{99.2} / 99.4 & \textbf{96.2} / 97.6 &          \textbf{93.1} / 96.6 & \textbf{89.3} / 96.0 &      84.7 / 95.5  \\
          \hline
         M& Middle (end-to-end), $|\mathcal{D}_3| = \frac{3N}{2}$  & \textbf{94.3} / 95.8  &82.1 / 90.9&          77.2 / 89.5&          73.0 / 88.2&          69.6 / 87.1 \\   
         N & Middle (end-to-end), $|\mathcal{D}_3| = N$  &          93.7 / 95.4 & 84.3 / 91.7 &          79.5 / 90.2 &          74.0 / 89.0 &      71.3 / 88.3 \\
          O  & Middle (nested), $|\mathcal{D}_{1,2,3}| = N$ &          94.2 / 94.7 &\textbf{87.3} / 91.2 &          \textbf{82.6} / 89.3 &          \textbf{77.7} / 88.5 &      \textbf{72.8} / 87.3  \\
          \hline
          P& Fine (end-to-end), $|\mathcal{D}_3| = \frac{3N}{2}$          & \textbf{88.3} / 91.5 &70.8 / 83.5 &          62.6 / 81.3 &          55.0 / 80.5 &          48.3 / 79.6     \\
          Q & Fine (end-to-end), $|\mathcal{D}_3| = N$ &          87.1 / 91.1 & 70.1 / 84.7 &          62.3 / 83.0 &          54.7 / 81.1 &      50.3 / 80.2 \\
            R &  Fine (nested), $|\mathcal{D}_{1,2,3}| = N$ &          86.7 / 87.9 &
            \textbf{73.7} / 81.3 &          \textbf{67.6} / 77.6 &          \textbf{57.6} / 76.4 &      \textbf{51.2} / 74.4  \\
          \hline
          \hline
        \multicolumn{7}{|c|}{MNIST}\\
          \hline
            S & Coarse (end-to-end), $|\mathcal{D}_3| = \frac{3N}{2}$  & 99.4 / 99.5 &   96.1 / 97.8 &          90.9 / 95.3 &          82.3 / 92.6 &          72.0 / 90.9   \\
            T & Coarse (nested), $|\mathcal{D}_{1,2,3}| = N$ &   \textbf{99.5} / 99.5 & \textbf{96.9} /  97.5&          \textbf{92.3} / 95.4&          \textbf{85.9} / 93.8&          \textbf{79.6} / 92.1   \\
            \hline
            U & Middle (end-to-end), $|\mathcal{D}_3| = \frac{3N}{2}$ & 99.1 /  99.2 & 94.8 / 96.9&          87.5 / 93.3&          74.6 / 89.8 &          60.7 / 88.0    \\
            V & Middle(nested), $|\mathcal{D}_{1,2,3}| = N$  & \textbf{99.2} / 99.2   & \textbf{95.5} / 96.0 &          \textbf{87.9} / 92.6 &          \textbf{77.0} / 89.4 &          \textbf{66.5} / 87.9 \\
            \hline
            W & Fine(end-to-end), $|\mathcal{D}_3| = \frac{3N}{2}$ &   98.5 / 98.7 &91.9 / 95.4&          80.4 / 90.9&          67.2 /  85.7 &          49.7 / 83.1      \\
            X &  Fine (nested), $|\mathcal{D}_{1,2,3}| = N$ &     \textbf{98.6}  / 98.4 &\textbf{92.8} /  93.5&          \textbf{82.8} / 87.8 &          \textbf{67.5} / 83.0  &          \textbf{50.6} / 80.4 \\
            \hline

\end{tabular}
\end{center}
    \caption{\footnotesize Complementary results of accuracy and mean confidence ($Acc\% / Conf\%$) for Fashion-MNIST, and MNIST datasets. In this experiments, we set $N = 6000$ Other results for Cifar 10, DBPEDIA, CIFAR100 and Plantvillage are reported in Table~\ref{tab:cifar10_202020vs20} and Table~\ref{tab:real_world_data}. }
    \label{app:tab:mnist_fmnist_202020vs20}
\end{table}

% ====================================================== %
% ====================================================== %
% ----------------------------------------------------------- %
\vspace{-10mm}
\subsection{Comparing with a common MTL architecture}\label{app:sec:MTL}
% ----------------------------------------------------------- %
%
A common Multi Task Learning (MTL) architecture consists of shared convolutional blocks followed by task-specific classification (fully connected) layers. 
%
Figure \ref{app:fig:new_architecture} illustrates an MTL architecture designed to obtain a nested classification of MNIST digits. 
%
The network enforces an information bottleneck that encodes the input into a (64,1) dimensional feature vector.
%
Then, it is connected to three classification branches implemented by a sequence of fully-connected layers.
%
This MTL model and our nested model have approximately the same number of parameters and are trained in an identical way on the MNIST dataset. 
\begin{figure}[htp]
    \centering
    \includegraphics[width = 0.8 \textwidth]{figures/architectureMTL.png}
    \caption{\footnotesize Architecture of the tested Multi-Task-Learning CNN. This architecture corresponds to a sequence of three blocks of two (convolutional + batch normalization) layers followed by a maxpooling layer. In order to reduce the dimension of the penultimate feature vector, we perform a global average pooling. This network and our nested CNN have approximately the same number of parameters and are trained using the same training protocol and data.}
    \label{app:fig:new_architecture}
\end{figure}
% ---
Table~\ref{app:tab:nested_vs_MTL} shows the classification accuracy for our nested architecture presented in Section \ref{app:sec:implem_details} and the Multi-Task Learning architecture presented above. 
%
On the original distribution both architectures perform roughly equivalently, but on perturbed test data the proposed nested model is considerably superior. 
%
Nested learning outperforms its MTL counterpart with a gap of 18\% for the fine task and a gap of more than 10\% for the coarse task for distortion levels 3 and 4. 
%
These results provide additional evidence that having a nested architecture promotes robustness and leads to more consistent models. 
% 
\begin{table}[ht]
\scriptsize
\centering
        \begin{tabular}{|c|c|c|c|c|c|c|}
        \hline
                  Method & Original & Distortion 1 &  Distortion 2 &  Distortion 3 &  Distortion 4 \\
        \hline
        \hline
             Coarse (MTL),$|\mathcal{D}_{1,2,3}| = N$  & 99.5 / 99.7 &         92.4 / 96.5 &          82.6 / 94.3 &          73.8 /92.9 &          66.1 / 93.1      \\
             Coarse (nested) Ours, $|\mathcal{D}_{1,2,3}| = N$ &   \textbf{99.5} / 99.5 &       \textbf{96.9} /  97.5&          \textbf{92.3} / 95.4&          \textbf{85.9} / 93.8&          \textbf{79.6} / 92.1      \\
             \hline
             Middle (MTL), $|\mathcal{D}_{1,2,3}| = N$ & 99.1 /  99.4 &         91.1 / 94.9&          75.5 / 90.8&          60.2 / 88.8 &          49.9 / 88.2     \\
             Middle (nested) Ours, $|\mathcal{D}_{1,2,3}| = N$  & \textbf{99.2} / 99.2   &      \textbf{95.5} / 96.0 &          \textbf{87.9} / 92.6 &          \textbf{77.0} / 89.4 &          \textbf{66.5} / 87.9 \\
             \hline
             Fine(MTL), $|\mathcal{D}_{1,2,3}| = N$ &   \textbf{98.9} / 99.0 &       91.0 / 89.9&          70.9 / 81.3&          48.6 /  77.9 &          32.4/ 80.1      \\
              Fine (nested) Ours, $|\mathcal{D}_{1,2,3}| = N$ &     98.6  / 98.4 &     \textbf{92.8} /  93.5&          \textbf{82.8} / 87.8 &          \textbf{67.5} / 83.0  &          \textbf{50.6} / 80.4    \\
        \hline
        \end{tabular}
    \caption{\footnotesize Classification accuracy and mean confidence ($Acc\% / Conf\%$) for an example of MTL and nested learning on the MNIST dataset. Coarse, fine, and middle indicate the accuracy at each level of the label. MTL denotes the standard Multi-Task Learning architecture described in Section~\ref{app:sec:MTL}, while ``nested'' denotes the proposed nested model. In this experiment we set $N=12000$.}
    \label{app:tab:nested_vs_MTL}
\end{table}

% ---
% ----------------------------------------------------------- %
\subsection{Skipped connections and their impact on the flow of information}\label{app:sec:skipedConnections}
% ----------------------------------------------------------- %
Obtaining an empirical measure of the mutual information (MI) between two high dimensional random variables is a very hard numerical problem \cite{paninski2003estimation}.
%
However, recent progresses in deep learning made a numerical approximation (MINE algorithm) tractable by exploiting the flexibility of neural networks and properties of the mutual information. 
%
Belghazi et al.~\cite{belghazi2018mine} showed that a the problem of estimating MI, can be formulated as an optimization problem. 
%
They rely on the following characterization of the mutual information between random variables $X$ and $Z$  as the Kullback-Leibler (KL) divergence :
\begin{equation}
    I(X,Z) = D_{KL}(\mathbb{P}_{XZ} || \mathbb{P}_X \otimes \mathbb{P}_Z).
\end{equation}
Based on this, the authors use the Donsker-Varadhan representation of the KL divergence, which introduces a dual optimization problem,
\begin{equation}\label{app:eq:MI_dual}
    D_{KL}(\mathbb{P}||\mathbb{Q}) = \sup_{T:\Omega \rightarrow \mathbb{R}} \mathbb{E}_{\mathbb{P}}[T] - \log(\mathbb{E}_{\mathbb{Q}}[e^{T}]),
\end{equation}
where the supremum is taken over all the functions $T$ for which both terms in the right side of the equation are finite.
% ---

Since the parameters of a neural network can be used to encode a large space of functions, the authors propose to solve Equation~\ref{app:eq:MI_dual} for $T_\theta \in \mathcal{F}$, where $\mathcal{F}$ denotes the space of functions encoded by a pre-defined network architecture with parameters $\theta\in\Theta$. 
%
An approximation of the MI can be obtained solving the problem
\begin{equation}\label{app:eq:MINE}
    I_{\Theta}(X,Z) = \sup_{\theta \in \Theta} \mathbb{E}_{\mathbb{P}_{XZ}}[T_{\theta}] - \log(\mathbb{E}_{\mathbb{Q}}[e^{T_{\theta}}]).
\end{equation}
%
Equation~\ref{app:eq:MINE} can be solved in practice using standard optimization tools of deep learning (see \cite{belghazi2018mine} for details).
% ---

In order to measure the impact of skipped-connections from an MI perspective, we measure the empirical approximation of the MI between different sections of the proposed nested architecture. 
%
We compared these results for the same network with and without skipped connections.
%
Let us refer to the network with skipped connections with the subscript 1 and the network without skipped connections with the subscript 2.
% ---

We define different variables of interest at particular stages of the network and estimate the mutual information between them.
%
We will refer as $F_1(X)$ and $F_2(X)$ the variable corresponding to the feature map created after the 2nd maxpooling layer with and without skipped connections (see figures \ref{app:fig:mnist_architecture} and 4). 
% 
Similarly, let $G_1(X)$ and $G_2(X)$ be the feature maps obtained before the second global average pooling (GAP) layer.
%
We will also consider $H_1(X)$ and $H_2(X)$ the coarsest feature maps obtained before the first GAP.
%
(Before feeding these features to the MINE algorithm we performed average pooling to reduce the dimension of the input variables.)
% ---

We estimated the MI between $I(F_i(X), G_i(X))$ and $I(F_i(X), H_i(X))$, $i=1$ meaning ``with skipped connections'' and $i=2$ ``without skipped connections''. (The network without skipped connections is re-trained to allow the model to adapt to this new configuration).  
% 
%We obtain the following measurements after 3000 iterations of MINE.
%\begin{align}
%    I(F_1(X),H_1(X)) &= 4.3, \\
%    I(F_2(X),H_2(X)) &= 3.7, \\
%    I(F_1(X),H_1(X)) &= 3.9, \\
%    I(F_2(X),H_2(X)) &= 3.5.
%\end{align}
%
Figure \ref{fig:MI} (left side) sketches in which sections of the model we are measuring the mutual information, and (right side) the evolution of the MI estimation (MINE algorithm) for $3000$ steps. 
%$$I(F_1(X),G_1(X)) = 4.3, I(F_2(X),G_2(X)) = 3.7 $$
% ---
\begin{align}\label{app:eq:results_mi}
    \Delta_1 = I(F_1(X),G_1(X))- I(F_1(X),H_1(X)) = 0.37, \\
    \Delta_2 = I(F_2(X),G_2(X))- I(F_2(X),H_2(X)) = 0.21 \approx{\Delta_1/2}.
\end{align}
%
As shown in equations 6 and 7 and discussed in Section 4, skipped connections play an important role to allow information to flow to the coarse feature representations of the finer representations. 
% 
This provides additional numerical evidence to the discussion presented in Section~\ref{sec:Theory} supporting the importance of including skipped connections and avoiding information bottleneck at the finer classification. 
% ---

% ====================================================== %
\section{Perturbations}\label{app:sec:perturbation}
\counterwithin{table}{section}
\counterwithin{figure}{section}
% ====================================================== %
Selecting realistic and meaningful perturbations to test DNN models is a non trivial problem. 
%
For example, adding Gaussian noise mainly affects the high frequency components of the input images and we observed that both standard end-to-end and nested networks are not affected by this type of perturbation.  
%
In this work we focus on structural deformations inspired by a model of turbulence. 
%
The pseudo-code of this perturbation is presented in Algorithm \ref{app:algo1} and was inspired by \cite{ipol_turbulence}.
%
Figure~\ref{app:fig:examples_distortion} illustrates the distortion of an example image from the MNIST dataset for different levels of \emph{turbulence intensity}.
%
\begin{figure}[htp]
    \centering
    \includegraphics[width = 0.19\textwidth]{figures/original_1.jpg}
    \includegraphics[width = 0.19\textwidth]{figures/warp075_1_1.jpg}
    \includegraphics[width = 0.19\textwidth]{figures/warp1_1_1.jpg}
    \includegraphics[width = 0.19\textwidth]{figures/warp125_1_1.jpg}
    \includegraphics[width = 0.19\textwidth]{figures/warp15_1_1.jpg}
    \caption{\footnotesize Example of different perturbations applied during testing time. From left to right: the original sample, and the distorted version with parameters $(S,T) = (1,0.8)$, $(S,T) = (1,1.0)$, $(S,T) = (1,1.3)$, and $(S,T) = (1,1.5)$ respectively.}
    \label{app:fig:examples_distortion}
\end{figure}
%
This perturbation is very helpful to test the robustness of neural networks as it affects the appearance, the edges, and morphology of the presented objects.  
%
\begin{algorithm}[htp]
\SetAlgoLined
\KwData{the input: $I\in \mathbb{R}^{w,h}$, the parameters $(S,T) \in \mathbb{R}^2$}
\KwResult{the distorted image $I_{dist}^{(S,T)}$}
Creating a vector field (u,v) for the distortion:\\
$u,v = normal\_noise((w,h)), normal\_noise((w,h))$\\
$u,v = gaussian\_filter(u,S), gaussian\_filter(v,S)$\\
$u,v = u\times \frac{T}{std(u)}, v\times \frac{T}{std(v)}$\\
Interpolate the image with the obtained vector field: \\
$I_{dist}^{(S,T)} = bilinear\_interpolate(I,u,v)$
\caption{Turbulence distortion}\label{app:algo1}
\end{algorithm}
% ---

\section{Geometry}\label{app:Geometry}
In addition to looking at the evolution of the accuracy during the cascaded training of our model in Section~\ref{sec:Experiments}, we also investigate the behaviour of some specific features of the network by visualizing their 2D-TSNE embedding.
%
This analysis is also extremely helpful to intuitively understand some of the results obtained in Section 5. 
%
For example, why our model is less sensitive to adversarial attacks, and why even when the fine label is misled the middle and coarse predictions remain rather accurate. 
% --

We chose to visualize the embedding of the features extracted by the global average pooling layers of the nested MNIST model and the end-to-end model. 
%
We do so at each of the three main steps of our training method for the nested model (i.e. training with coarse annotations only first, training with coarse and middle annotations, and finally training on coarse middle and fine annotations) and after 50 and 100 epochs for the end-to-end model.
% ---

As we can see in Figure~\ref{app:fig:geometry}, the feature embedding of the nested model have a much more reasonable structure than the end-to-end model. 
%
This makes sense, as end-to-end learning tries to find a representation that separates different classes, but there is no explicit reward to map similar classes closer to each other.
%
On the other hand, nested learning encourages a nested representation as we can see in Figure G.1, from all the possible solutions that separate the fine classes, our model is choosing one that maps together fine classes with nested similarities.
% ---

%
If we look at the evolution of the feature embeddings, we can clearly identify clusters, which correspond to coarse middle and fine classes as we introduce more than one level of annotation, whereas the data points are almost distributed uniformly for the end-to-end model. 
%
Even though the accuracy of the fine predictions are similar, the feature embedding of our model shows a better and more natural 2D structure, with fine classes of the same middle class being close to each other. For example, the samples from classes 4, 7, and 9 -which belong to the same intermediate class- are close to each other in the 2-D embedding of the features extracted by the last GAP layer.
%
\begin{figure}
    \centering
    \includegraphics[width = \textwidth]{eccv2020kit/figures/NestedLearning2D.png}
    \caption{2D feature embedding for nested versus end-to-end learning. From left to right, we see how the feature embedding evolves as training proceeds. The first row shows the feature embedding of the features prior the coarse prediction, the middle row the embedding associated to the middle prediction, and finally, the last row the embedding associated to the fine prediction. On the right side, we compare the feature embedding for the fine prediction trained in an end-to-end fashion.}
    \label{app:fig:geometry}
\end{figure}


